BALI: Learning Neural Networks via Bayesian Layerwise Inference

We introduce a new method for learning Bayesian neural networks, treating them as a stack of multivariate Bayesian linear regression models. The main idea is to infer the layerwise posterior exactly if we know the target outputs of each layer. We define these pseudo-targets as the layer outputs from the forward pass, updated by the backpropagated gradients of the objective function. The resulting layerwise posterior is a matrix-normal distribution with a Kronecker-factorized covariance matrix, which can be efficiently inverted. Our method extends to the stochastic mini-batch setting using an exponential moving average over natural-parameter terms, thus gradually forgetting older data. The method converges in few iterations and performs as well as or better than leading Bayesian neural network methods on various regression, classification, and out-of-distribution detection benchmarks.

==> sec/outdated_stuff.tex <==
\subsection{Multi-output Bayesian linear regression}\label{sec:background:multioutput_linear_regression}
% Next, we consider the case when multiple targets are predicted from the same inputs. 
% This can be modeled with a distinct set of weights and a linear transformation:
Next, we consider the case when multiple targets are linearly predicted from the same inputs and a distinct set of weights:
\begin{align}\label{eq:multioutput_single_obs}
\by_n = W^T \bx_n + \boldsymbol{\epsilon}_n, ~~~~~ \boldsymbol{\epsilon}_n \sim \mathcal{N}(0, \Sigma),
\end{align}
where $\bz_n = W^T \bx_n$ is the prediction resulting from the linear transformation of the inputs $\bx_{n} \in \mathbb{R}^{D_i}$ with the weight matrix $W \in \mathbb{R}^{D_i \times D_o}$, and $\Sigma \in \mathbb{R}^{D_o \times D_o}$ is the noise covariance of the likelihood. 


% Thus, considering a batch of $N$ inputs and targets with independent noise, the multi-output linear model prediction is given by
% \begin{align}
% Y = X W^T + \boldsymbol{\epsilon}, ~~~~~ \boldsymbol{\epsilon} = [\boldsymbol{\epsilon}_1, \, \dots, \, \boldsymbol{\epsilon}_N]^T, %,~~~ \epsilon_n \sim \mathcal{N}(0, \Sigma_n).
% \end{align}
% where $X \in \mathbb{R}^{N \times D_i}$ as in Sec.~\ref{sec:background:univariate_linear_regression}, and the targets $Y \in \mathbb{R}^{N \times D_o}$ are now also matrix-valued. 


In order to define the posterior distribution, it is helpful to rewrite the model using vectorised weights, $\weights := \mathrm{vec}(W)$, concatenating the columns of the weight matrix, each corresponding to weights connected to the same output node.
The likelihood is then given by
\begin{align}
    p(Y | X, \weights) &= \prod_{n=1}^{N} p(\by_n | \bx_n, \weights), \\
    p(\by_n | \bx_n, \weights) &= \mathcal{N}(\by; \underbrace{(\mathbf{I}_{D_o} \kron \bx_n^T)}_{\bar{X}_n}  \weights, \Sigma).
\end{align}
where $X \in \mathbb{R}^{N \times D_i}$ and $Y \in \mathbb{R}^{N \times D_o}$ are a batch of $N$ inputs and corresponding targets, respectively. 
The vectorisation of the linear transformation in \eqref{eq:multioutput_single_obs} leads to a Kronecker product between an input vector $\bx_n$ and the identity matrix $\mathbf{I}_{D_o}$ of size $D_o$, which we denote by $\bar{X}_n \in \mathbb{R}^{D_o \times D_o \cdot D_i}$. 
With this formulation, the per-data likelihood with $D_o$-dimensional targets has the same form as the univariate likelihood with $N$ data points (cf.~\eqref{eq:univariate_likelihood}).
Taking the product between the prior and the $N$ likelihood terms, the posterior is thus Gaussian with the following natural parameters:
\begin{subequations}\label{eq:multioutput_natural_params_general}
\begin{align}
V^{-1} &= V_0^{-1} + \sum_{n=1}^N \bar{X}^T_n \Sigma^{-1} \bar{X}_n \\
\boldsymbol{\eta} &= V_0^{-1} \bm_0 + \sum_{n=1}^N \bar{X}^T_n \Sigma^{-1} \by_n.
\end{align}
\end{subequations}
Since the inputs $\bar{X}_n$ of the vectorised model have a Kronecker-product structure, we can write the natural parameters from \eqref{eq:multioutput_natural_params_general} in a more compact form.
To this end, define the \emph{matrix} of weight prior means by $M_0 \in \mathbb{R}^{D_i \times D_o}$ such that $\bm_0 = \textrm{vec}(M_0)$.
Furthermore, consider a Gaussian prior with a Kronecker-factorised covariance\footnote{A Gaussian distribution over the elements of a matrix with a Kronecker-factorised covariance matrix is also referred to as a Matrix-Normal distribution.} 
\begin{equation}
    V_0 = S_0 \kron R_0.
\end{equation}
% where $\bs_o \in \mathbb{R}^{D_o}$ are scale factors per each output node and $\bs_i \in \mathbb{R}^{D_i}$ are scales corresponding to input nodes. 
% The prior natural parameters can then be computed as (cf.~\ref{app:kfac_approx})
% \begin{align}
%     V_0^{-1} &= (S_0 \kron R_0)^{-1} = S_0^{-1} \kron R_0^{-1}, \\
%     \boldsymbol{\eta}_0 &= V_0^{-1} \bm_0 = \textrm{vec}(R_0 M_0 S_0).
% \end{align} 
% and the posterior natural parameters can be computed as (cf.~\ref{app:kfac_approx})
% Since the inputs $\bar{X}_n$ of the vectorised model have a Kronecker-product structure, we can write the natural parameters from \eqref{eq:multioutput_natural_params_general} in a more compact form (cf.~App.~\ref{app:kfac_approx}):
The posterior natural parameters can then be computed as (cf.~\ref{app:kfac_approx})
\begin{subequations}\label{eq:natural_params_kron}
\begin{align}
V^{-1} &= \overbrace{S_0^{-1} \kron R_0^{-1}}^{V_0^{-1}} + \overbrace{\Sigma^{-1} \kron X^T X}^{V_{1:N}^{-1}}, \label{eq:precision_kron}\\
\Eta &= \underbrace{R_0 M_0 S_0^T}_{\Eta_0} + \underbrace{X^T Y \Sigma^{-1}}_{\Eta_{1:N}}, \label{eq:eta_kron}
\end{align}
\end{subequations}
where $\Eta \in \mathbb{R}^{D_i \times D_o}$ denotes the \emph{matrix} of precision-means such that $\boldsymbol{\eta} = \mathrm{vec}(\Eta)$. 
% where $M_0 \in \mathbb{R}^{D_i \times D_o}$ is the prior mean \emph{matrix} and $\Eta \in \mathbb{R}^{D_i \times D_o}$ is the posterior precision-mean \emph{matrix}, where these matrices conveniently have the shape of the weight matrix. 












\subsection{Layerwise posterior approximation}\label{sec:method:posterior}
The pseudo-targets defined in \eqref{eq:pseudo_targets} by definition have a higher likelihood than the layer outputs from the forward pass (for a small enough step size $\beta$).
However, rather than using backpropagation one step further to update a maximum likelihood \emph{point estimate} of the weights, we use $\by_{n,l}$ to infer the \emph{posterior distribution} of the multi-output Bayesian linear regression model (cf.~Sec.~\ref{sec:background:multioutput_linear_regression}) in layer $l$. 

We assume that the prior is independent over each layer, and, similarly, consider a layerwise posterior approximation that factorises over layers. 
In the following, we therefore drop the layer indices $l$ for notational convenience. 
We assume that the layerwise prior is a Gaussian distribution with a Kronecker-factorised diagonal covariance
\begin{equation}\label{eq:kron_prior_cov:definition}
    V_0 = S_0 \kron R_0 = \mathrm{Diag} \left( \bs_0 \right) \kron \mathrm{Diag} \left( \br_0 \right),
\end{equation}
where $\bs_0 \in \mathbb{R}^{D_o}$ are scale factors per each output node and $\br_0 \in \mathbb{R}^{D_i}$ are scales corresponding to input nodes. 
Using the pseudo-targets from Sec.~\ref{sec:method:targets}, we also define a \emph{pseudo-likelihood} as
\begin{align}\label{eq:pseudo-likelihood}
    p(\by_{n} | \bx_{n}) = \mathcal{N}(\by_{n}; \bar{X}_{n} \weights_{t}, \Sigma),
\end{align}
where $\bar{X}_{n} \weights_{t} = W^T_{t} \bx_{n}$ is the linear transformation with a weight sample at iteration $t$, $\bar{X}_{n} = \mathbf{I}_{D_{o}} \kron \bx_{n}^T$ analogous to the multi-output Bayesian linear regression model in Sec.~\ref{sec:background:multioutput_linear_regression}, and $\Sigma = \text{Diag}(\boldsymbol{\sigma}^{2})$ is the noise covariance matrix (in layer $l$).


% The posterior mean is computed by $\bm = V \boldsymbol{\eta}$ and the covariance matrix $V$ requires a matrix inversion that generally has a computational complexity of the order $O\big((D_o \cdot D_i)^3 \big)$.

% We assume a prior distribution that factorises over each layer and has a Matrix-Normal distribution per layer.
% \TODO{layer index missing. Maybe good to do this without. Should it be in this section then though?}
% \begin{align}
%     p(\weights) = \prod_{l=1}^{L} \mathcal{MN}(\weights; M_0, V_0^i, V_0^o)
% \end{align}





% The posterior of this model is a Gaussian with natural parameters
% \begin{align}\label{eq:multioutput_natural_params_general}
% V^{-1} &= V_0^{-1} + \sum_{n=1}^N \bar{X}^T_n \Sigma_n^{-1} \bar{X}_n, \\
% \boldsymbol{\eta} &= V_0^{-1} \bm_0 + \sum_{n=1}^N \bar{X}^T_n \Sigma_n^{-1} \by_n.
% \end{align}
% Due to the Kronecker-product structure, we can simplify the precision terms stemming from the likelihood (cf.~App.~\ref{sec:appendix:kronecker}):
% \begin{align}\label{eq:kronecker_data_terms}
% \bar{X}_n \Sigma_n^{-1} \bar{X}_n^T
% &= \Sigma_n^{-1} \kron (\bx_n \bx_n^T).
% \end{align}
% Similarly, the block-wise updates to the precision-mean are
% \begin{align}
%     \bar{X}^T_n \Sigma_n^{-1} \by_n &=  \text{vec}\left( \Sigma^{-1}_n \by_n \bx^T_n \right),
% \end{align}
% where the precision-mean matrix inside the vectorisation operator has the same shape as the weight matrix.



The posterior of this layerwise Bayesian linear regression model is a Gaussian with natural parameters given by \eqref{eq:natural_params_kron}. 
Despite the compact structure using Kronecker products, inverting the precision matrix has a computational complexity of the order $O\big((D_o \cdot D_{i})^3 \big)$. 
This is because the sum of the two Kronecker products is generally not a Kronecker product. 
Similar to the Kronecker-factored Approximate Curvature (KFAC) in \cite{Martens2015KFAC} used in the context of natural gradient descent, we approximate the posterior precision matrix using the following Kronecker-product structure (cf.~App.~\ref{app:kfac_approx}):
\begin{align}\label{eq:kron_precision}
V^{-1}
& \approx
\left( N^{-1} \cdot S_0  + \Sigma^{-1} \right) 
\kron 
\left( R_0 + X^T X \right),
\end{align}
where $N$ is the dataset size, and $\Eta = R_0 M_0 S_0^T + X^T Y \Sigma^{-1}$ as in \eqref{eq:natural_params_kron}, requiring no further approximation.

The posterior mean and variance can then be computed efficiently as (cf.~App.~\ref{app:kfac_approx})
\begin{subequations}\label{eq:kron_mean_var}
\begin{align}
V & \approx
\left( N^{-1} \cdot S_0  + \Sigma^{-1} \right)^{-1}
\kron 
\left( R_0 + X^T X \right)^{-1}, \\
M &= \left( R_0 + X^T X \right) \Eta \left( N^{-1} \cdot S_0  + \Sigma^{-1} \right),
\end{align}
\end{subequations}
where the approximation for $V$ is again due to the Kronecker-product approximation in \eqref{eq:kron_precision}. 

We sample from this distribution by first drawing $D_i \cdot D_o$ samples from a standard normal distribution, $\boldsymbol{\nu} \sim \mathcal{N}(\mathbf{0}, \mathbf{1})$, and then transform these samples by the cholesky factors 
\begin{align}
    \weights_t &= 
    \left( N^{-1} \cdot S_0  + \Sigma^{-1} \right)^{\frac{1}{2}}
    \mathrm{Diag}(\boldsymbol{\nu})
    \left( R_0 + X^T X \right)^{\frac{1}{2}}.
\end{align}


Note that computing the posterior parameters, the layerwise posterior-predictive distribution and sampling from this posterior each has a computational complexity that is not greater than $O(D_i^3 + D_o^3 + D_i^2 \cdot D_o + D_i \cdot D_o^2)$, since the matrix can be inverted efficiently via $(A \kron B)^{-1} = A^{-1} \kron B^{-1}$ and the matrices involved in the computation of the means are each only of size $D_i$ or $D_o$. 









\section{Kronecker-factorised posterior approximation}\label{app:kfac_approx}
Inverting the posterior precision matrix $V^{-1} \in \mathbb{R}^{D_o \cdot D_i \times D_o \cdot D_i}$ from \eqref{eq:multioutput_natural_params_general} is in general of the order $O((D_o \cdot D_i)^3)$. 
If we assume that all prediction errors are independent also among the $D_o$ output dimensions, the model reduces to $D_o$ independent univariate Bayesian linear regression models, where we have to perform $D_o$ matrix inversions, resulting in the computation complexity of the order $O(D_o \cdot D_i^{3})$. 
On the other hand, full noise covariance matrices $\Sigma_n$ render the posterior over weights corresponding to different outputs dependent. 


The computational cost may not play a role in many linear regression settings, where we have only few inputs and targets and where we have to do the matrix inversion only once. 
However, if both $D_o$ and $D_i$ are large and we have to do many such updates as part of an iterative learning algorithm, such a computational cost is infeasible.  
In order to drastically reduce the computational cost, the KFAC approximation has been proposed as an efficient approximation of the Fisher matrix in the context of natural gradient descent \cite{Martens2015KFAC, noisyKFAC, others} and the Laplace approximation \cite{LaplaceRedux, theNewOne, others} for neural networks. 
KFAC approximates the average of Kronecker products by a Kronecker product of averages.
In the context of multi-output Bayesian linear regression models with heteroscedastic noise, this corresponds to 
\begin{align}
V^{-1}_{1:N} = \sum_{n=1}^N \Sigma_n^{-1} \kron \left( \bx_n \bx_n^T \right)
 & \approx \frac{1}{N} \cdot \sum_{n=1}^N \Sigma_n^{-1} \otimes \sum_{n=1}^N \bx_n \bx_n^T.
\end{align}
In our layerwise Bayesian linear regression model, we assume a homoscedastic noise distribution, i.e., $\forall n: \Sigma_n = \Sigma$. 
Hence, for this part, we do not require an approximation to maintain the form of a Kronecker product, since we can simply pull out the covariance matrix from the sum and obtain
\begin{align}
V^{-1}_{1:N} = \sum_{n=1}^N \Sigma^{-1} \kron \left( \bx_n \bx_n^T \right)
 & =\Sigma^{-1} \otimes \sum_{n=1}^N \bx_n \bx_n^T.
\end{align}
Unfortunately, when adding the prior precision to the above term to obtain the posterior precision, the Kronecker product structure is lost in general. 
However, since we have a Kronecker-product structured prior covariance, we can use the approximation of \cite{Martens2015KFAC} for the sum of the prior and data term. 
With the Kronecker-factored prior precision, the Kronecker-factorised approximation of the posterior precision is
\begin{align}
V^{-1} 
&= S_0^{-1} \kron R_0^{-1}  + \Sigma_n^{-1} \kron \sum_{n=1}^{N} \bx_n \bx_n^T \\
&= N \cdot \frac{1}{N} \left( S_0^{-1} \kron R_0^{-1}  + \sum_{n=1}^{N} \Sigma_n^{-1} \kron  \bx_n \bx_n^T \right) \\
& \approx N \cdot \frac{1}{N }\left( S_0^{-1} + N \cdot \Sigma^{-1} \right) \kron \frac{1}{N} \left(R_0^{-1} + \sum_{n=1}^{N} \bx_n \bx_n^T \right) \\
& = \left(\frac{1}{N} S_0^{-1} + \Sigma^{-1} \right) \kron \left(R_0^{-1} + X^T X \right), 
\end{align}
where we used $\frac{1}{N}$ rather than $\frac{1}{N+1}$ for simplicity, as in \cite{Martens2015KFAC}.
%
Note that we could have also used the reparametrised prior scales $\hat{S}_o^{-1} =  \alpha \cdot S_0^{-1}$ and $\hat{S}_i^{-1} =  \alpha^{-1} \cdot S_0^{-1}$ for any positive scalar $\alpha$, e.g.\ with $\alpha = \sqrt{N}$, because
\begin{align}
    V_0^{-1} = S_0^{-1} \kron R_0^{-1} = (\alpha \cdot S_0^{-1}) \kron (\alpha^{-1} \cdot R_0^{-1}).
\end{align}
However, since we optimise the parameters $S_0$ and $R_0$, specifying an additional hyper-parameter $\alpha$ would be unnecessary. 
% Inverting the KFAC precision matrix is only of the order $O(D_o^{3} + D_i^{3})$ rather than $O(D_o^{3} \cdot D_i^{3})$ for inverting the precision matrix without approximation. 



Using the inverse property \ref{thm:kronecker:inverse}, the posterior covariance matrix is given by
\begin{align}
V & = \left(\frac{1}{N} S_0^{-1} + \Sigma^{-1} \right)^{-1} \kron \left(R_0^{-1} + X^T X \right)^{-1}. 
\end{align}
Finally, we compute the posterior means $\bm$ in vectorised form and $M$ in matrix form, respectively. 
Using property \ref{thm:kronecker:Vectorisation}, we obtain
\begin{align}
\bm = V \boldsymbol{\eta} 
&= \left(\left( N^{-1} \cdot S_0^{-1}  + \Sigma^{-1} \right)^{-1} \kron \left( R_0^{-1} + X^T X \right)^{-1} \right) \mathrm{vec}\left(\Eta \right) \\
    &= \mathrm{vec}\left( \left(R_0^{-1} + X^T X \right)^{-1} \Eta \left( N^{-1} \cdot S_0^{-1}  + \Sigma^{-1} \right)^{-1} \right),
\end{align}
where we directly used $(N^{-1} \cdot  S_0^{-1}  + \Sigma^{-1})^{-T} = (N^{-1} \cdot  S_0^{-1}  + \Sigma^{-1})^{-1}$ since the matrix is symmetric. 
From the posterior means in vectorised form, we can directly read of the posterior means in matrix form as
\begin{align}
M = \left( R_0^{-1} + X^T X \right)^{-1} \Eta \left( N^{-1} \cdot S_0^{-1}  + \Sigma^{-1} \right)^{-1}.
\end{align}

